Unifying Score and Performance for Fine-Grained Music Understanding in Audio-Language Models

Large audio language models (LALMs) have shown promising progress in broad music-understanding tasks such as tagging, retrieval, and captioning. Music understanding that requires finer hearing over both the content and how it is realized within a performance through dynamics, phrasing, articulation, time, and other performance techniques, however, remains at an earlier stage. Existing audio-language model (ALM) training pipelines typically rely on coarse, weakly grounded captions and therefore provide little support for learning these subtle nuances in music, limiting their ability to serve real-world applications in education or artistic practice. We therefore introduce MuNo-SP (Music Notation unifying Score and Performance), a text-based representation that jointly encodes score content and performance information. Building on MuNo-SP, we develop an automatic training-data generation pipeline that uses aligned scores and performances to produce long-form auditory analyses and musically informed question-answer pairs. We use this pipeline to construct MAESTROCaps, a classical piano dataset comprising 148 long-form performance analyses and 31,080 question-answer pairs derived from 148 aligned score-performance pairs. In a human evaluation, MuNo-SP analyses were preferred by majority vote over MIDI-only analyses for eight of nine excerpts. MuNo-SP also performed strongly on a benchmark of score-performance understanding, suggesting that integrating score and performance information enables more reliable and musically informative LALM supervision than a MIDI-only baseline.

==> results-table-musp.tex <==
% Requires: booktabs, multirow, graphicx, caption, xcolor
\providecommand{\result}[2]{}
\renewcommand{\result}[2]{#1\,{\scriptsize\textcolor{black!45}{[#2]}}}
\providecommand{\notapp}{}
\renewcommand{\notapp}{\textcolor{black!45}{\textnormal{N/A}}}
\providecommand{\notrun}{}
\renewcommand{\notrun}{\textcolor{black!45}{\textnormal{---}}}
\providecommand{\partialrun}{}
\renewcommand{\partialrun}{\textcolor{black!45}{\textnormal{partial}}}

\begin{table*}[t]
\centering


\fontsize{6.5}{7.2}\selectfont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llrccc@{}}
\toprule
\textbf{Subset} &
\textbf{Input} &
\textbf{\#Q} &
\shortstack{\textbf{GPT-5.6}\\\textbf{Sol}} &
\shortstack{\textbf{MuseSpark}\\\textbf{1.2}} &
\shortstack{\textbf{Qwen-3.6}\\\textbf{Plus}} \\
\specialrule{0.10em}{0pt}{0.7pt}

\multirow{4}{*}{Score only (S)}
& ABC
& 180
& \textbf{50.6}
& 31.7
& 11.1 \\

& Image
& 180
& \textbf{26.1}
& 15.0
& 13.3 \\

\cmidrule(lr){2-6}

& MuNo-S
& 180
& \textbf{\underline{83.3}}
& 65.6
& 20.6 \\

& MuNo-P
& 180
& \textbf{83.3}
& 62.8
& 15.6 \\

\specialrule{0.10em}{1.5pt}{0.7pt}

\multirow{2}{*}{Performance only (P)}
& MIDI-as-text
& 106
& \textbf{59.4}
& 30.2
& 10.4 \\

\cmidrule(lr){2-6}

& MuNo-P
& 106
& \textbf{\underline{77.4}}
& 57.5
& 22.6 \\

\specialrule{0.10em}{1.5pt}{0.7pt}

\multirow{2}{*}{\shortstack[l]{Score and\\performance (SP)}}
& ABC+MIDI
& 72
& \textbf{45.8}
& 30.6
& 6.9 \\

\cmidrule(lr){2-6}

& MuNo-P
& 72
& \textbf{\underline{80.6}}
& 52.8
& 20.8 \\

\specialrule{0.10em}{1.5pt}{0.7pt}

\multirow{5}{*}{\shortstack[l]{General\\(S/P)}}
& ABC
& 84
& \textbf{63.1}
& 53.6
& 33.3 \\

& MIDI-as-text
& 84
& \textbf{63.1}
& 46.4
& 23.8 \\

& Image
& 84
& 47.6
& \textbf{53.6}
& 35.7 \\

\cmidrule(lr){2-6}

& MuNo-S
& 84
& \textbf{78.6}
& 67.9
& 40.5 \\

& MuNo-P
& 84
& \textbf{\underline{79.8}}
& 66.7
& 42.9 \\

\specialrule{0.14em}{2pt}{1.2pt}

\multirow{4}{*}{\shortstack[l]{Score-available\\comparison}}
& ABC
& 264
& \textbf{54.5}
& 38.6
& 18.2 \\

& Image
& 264
& \textbf{33.0}
& 27.3
& 20.5 \\

& MuNo-S
& 264
& \textbf{81.8}
& 66.3
& 26.9 \\

& MuNo-P
& 264
& \textbf{\underline{82.2}}
& 64.0
& 24.2 \\

\specialrule{0.10em}{1.5pt}{0.7pt}

\multirow{2}{*}{\shortstack[l]{Performance-text\\comparison}}
& MIDI-as-text
& 190
& \textbf{61.1}
& 37.4
& 16.3 \\

& MuNo-P
& 190
& \textbf{\underline{78.4}}
& 61.6
& 31.6 \\

\specialrule{0.10em}{1.5pt}{0.7pt}

\multirow{2}{*}{\shortstack[l]{Joint score--performance\\comparison}}
& ABC+MIDI
& 72
& \textbf{45.8}
& 30.6
& 6.9 \\

& MuNo-P
& 72
& \textbf{\underline{80.6}}
& 52.8
& 20.8 \\

\specialrule{0.14em}{2pt}{1.2pt}

\multirow{4}{*}{Aggregate scores}
& Baseline mean
& 4 subsets
& \textbf{\underline{50.4}}
& 33.8
& 15.1 \\

& Baseline best
& 4 subsets
& \textbf{\underline{54.7}}
& 36.5
& 16.6 \\

\cmidrule(lr){2-6}

& MuNo mean
& 4 subsets
& \textbf{\underline{80.1}}
& 60.4
& 25.8 \\

& MuNo best
& 4 subsets
& \textbf{\underline{80.3}}
& 60.9
& 26.7 \\

\bottomrule
\end{tabular*}

\caption{Accuracy (\%) by question subset, input representation, and model.
The General (S/P) subset combines the general and tonality/style questions from the benchmark.
We exclude composer/work identification questions since the training pipeline will have access to it. 
Matched-coverage comparisons use identical question sets. Baseline and MuNo
means first average the available representations within each subset and then
average equally across the four included subsets; best scores use the strongest
representation in each subset.}
\label{tab:main-results}
\end{table*}
